Learning Graph Structures and Uncertainty for Accurate and Calibrated Time-series Forecasting

Multi-variate time series forecasting is an important problem with a wide range of applications. Recent works model the relations between time-series as graphs and have shown that propagating information over the relation graph can improve time series forecasting. However, in many cases, relational information is not available or is noisy and reliable. Moreover, most works ignore the underlying uncertainty of time-series both for structure learning and deriving the forecasts resulting in the structure not capturing the uncertainty resulting in forecast distributions with poor uncertainty estimates. We tackle this challenge and introduce STOIC, that leverages stochastic correlations between time-series to learn underlying structure between time-series and to provide well-calibrated and accurate forecasts. Over a wide-range of benchmark datasets STOIC provides around 16% more accurate and 14% better-calibrated forecasts. STOIC also shows better adaptation to noise in data during inference and captures important and useful relational information in various benchmarks.

==> Tables/forecast_full.tex <==
\begin{table*}[!ht]
\centering
\caption{Average Evaluation Scores (over 20 runs) for \model, baselines and ablation variants. The best-performing scores are in bold and the second-best is underlined. \model provides around 9\%, 14.7\%, and 16\% better performance in terms of RMSE, CS and CRPS respectively.}
\scalebox{0.99}{
\begin{tabular}{c|ccc|ccc|ccc|ccc}
             & \multicolumn{3}{c}{\flu}              & \multicolumn{3}{c}{\covid}                  & \multicolumn{3}{c}{\stocks}                     & \multicolumn{3}{c}{\power}                 \\ \hline
             & RMSE          & CRPS          & CS            & RMSE          & CRPS          & CS            & RMSE          & CRPS          & CS            & RMSE           & CRPS           & CS            \\ \hline
ARIMA       & 0.85          & 0.91          & 0.22          & 91.5          & 87.4          & 0.21          & 0.42          & 0.40          & 0.27          & 395.2          & 417.2          & 0.37          \\
\deepar       & 0.68          & 0.97          & 0.15          & 49.1          & 48.5          & \textbf{0.19}          & 0.35          & 0.41          & 0.18          & 249.9          & 267.8          & 0.18          \\
\tsfnp        & 0.64          & \underline{0.52}          & \textbf{0.05}          & 43.6          & 44.5          & 0.15          & 0.22          & 0.28          & \underline{0.16}          & 257.3          & 277.0          & 0.15          \\
MTGNN        & 0.68          & 0.75          & 0.18          & 48.3          & 49.5          & 0.22          & 0.17          & 0.26          & 0.19          & \textbf{189.3} & \textbf{207.1} & 0\underline{0.13}          \\
GDN          & 0.73          & 0.71          & 0.15          & 42.74         & 43.2          & 0.25          & 0.18          & 0.24          & 0.24          & 249.1          & 263.6          & 0.21          \\
\nir          & 0.71          & 0.74          & 0.22          & 63.44         & 72.19         & 0.35          & \underline{0.14}          & 0.23          & 0.19          & 315.9          & 338.6          & 0.18          \\
GTS          & \underline{0.63}          & 0.66          & 0.17          & \underline{41.96}         & \underline{36.25}         & 0.22          & \textbf{0.11} & 0.18          & 0.22          & 197.4          & 208.0          & 0.16          \\
LDS          & 0.69          & 0.64          & 0.16          & 45.17         & 41.32         & 0.23          & 0.15          & 0.19          & \underline{0.16}          & 213.6          & 229.0          & 0.19          \\ \hline
\model         & \textbf{0.57} & \textbf{0.42} & \underline{0.07} & \textbf{32.7} & \textbf{31.7} & \underline{0.2}  & \textbf{0.11} & \textbf{0.16} & \textbf{0.12} & \underline{191.6} & \underline{207.3} & \textbf{0.09} \\
\modelng & 0.67          & 0.51          & 0.06          & 42.7          & 41.6          & 0.11          & 0.24          & 0.31          & 0.16          & 226.5          & 248.5          & 0.13          \\
\modelns   & 0.65          & 0.68          & 0.15          & 44.72         & 40.66         & 0.19          & 0.12          & 0.21          & 0.15          & 196.4          & 211.0          & 0.11          \\
\modelnc  & 0.63          & 0.44          & 0.06          & {31.6} & {28.3} & {0.19} & 0.13          & 0.19          & 0.18          & 217.5          & 237.6          & 0.18          \\ \hline \hline
             & \multicolumn{3}{c}{\trafficla}                   & \multicolumn{3}{c}{\trafficbay}                 & \multicolumn{3}{c}{\nycb}                  & \multicolumn{3}{c}{\nyct}                    \\ \hline
             & RMSE          & CRPS          & CS            & RMSE          & CRPS          & CS            & RMSE          & CRPS          & CS            & RMSE           & CRPS           & CS            \\ \hline
ARIMA       & 2.17         & 2.06          & 0.23          & 4.1           & 3.9           & 0.14          & 4.27          & 4.11          & 0.34          & 18.55          & 17.49          & 0.15          \\
\deepar       & 2.05          & 1.93          & 0.17          & 3.8           & 4.2           & 0.16          & 3.11          & 3.15          & 0.28          & 14.52          & 15.77          & 0.17          \\
\tsfnp        & 2.11          & 1.89          & 0.14          & 4.1           & 3.9           & 0.13          & 2.94          & 2.85          & 0.23          & 15.13          & 14.97          & 0.15          \\
MTGNN        & \underline{1.86}          & 1.64          & 0.14          & \underline{3.2}           & \underline{2.9}           & \underline{0.11}          & 2.62          & \underline{2.61}          & \underline{0.17}          & \underline{10.37}          & \underline{10.13}          & \underline{0.13}          \\
GDN          & 1.95          & 1.83          & 0.16          & 3.4           & 3.1           & 0.16          & 2.74          & 1.78          & \textbf{0.15}          & 11.15          & 10.64          & 0.17          \\
\nir          & 2.17          & 1.95          & 0.19          & 7.9           & 5.3           & 0.14          & 3.18          & 4.7           & 0.36          & 14.38          & 17.52          & 0.31          \\
GTS          & 1.88          & \underline{1.74}          & 0.15          & 3.7           & 3.2           & 0.13          & 2.76          & 2.85          & 0.24          & 10.75          & 12.68          & 0.18          \\
LDS          & 2.12          & 2.05          & \underline{0.13}          & 3.5           & 3.7           & 0.18          & \underline{2.55}          & 2.67          & 0.21          & 11.44          & 13.98          & 0.19          \\ \hline
\model         & \textbf{1.84} & \textbf{1.48} & \textbf{0.11} & \textbf{2.8}  & \textbf{2.5}  & \textbf{0.08} & \textbf{2.52} & \textbf{2.41} & \textbf{0.15} & \textbf{8.43}  & \textbf{8.61}  & \textbf{0.09} \\
\modelng & 2.19          & 1.85          & 0.17          & 3.9           & 4             & 0.15          & 3.41          & 3.16          & 0.19          & 13.65          & 12.89          & 0.21          \\
\modelns   & 2.25          & 2.18          & 0.15          & 3.4           & 3.1           & 0.12          & 2.86          & 2.72          & 0.17          & 10.53          & 9.24           & 0.14          \\
\modelnc  & 1.86          & 1.54          & 0.14          & 3.7           & 3.6           & 0.09          & 2.95          & 2.69          & 0.21          & 9.25           & 8.37           & 0.11         
\end{tabular}
}
\label{tab:forecast}
\end{table*}

==> acks.tex <==
\par \noindent \textbf{Acknowledgments:} This work was supported in part by the NSF (Expeditions CCF-1918770,
CAREER IIS-2028586, RAPID IIS-2027862, Medium IIS-1955883, Medium IIS-2106961,
CCF-2115126, Small III-2008334), CDC MInD program, ORNL, ONR MURI
N00014-17-1-2656, faculty research awards from Facebook, Google and Amazon and
funds/computing resources from Georgia Tech.


==> exrelated.tex <==
\section{Additional Related works}

